CodeFuse-13B: A Pretrained Multi-lingual Code Large Language Model

Code Large Language Models (Code LLMs) have gained significant attention in the industry due to their wide applications in the full lifecycle of software engineering. However, the effectiveness of existing models in understanding non-English inputs for multi-lingual code-related tasks is still far from well studied. This paper introduces CodeFuse-13B, an open-sourced pre-trained code LLM. It is specifically designed for code-related tasks with both English and Chinese prompts and supports over 40 programming languages. CodeFuse achieves its effectiveness by utilizing a high quality pre-training dataset that is carefully filtered by program analyzers and optimized during the training process. Extensive experiments are conducted using real-world usage scenarios, the industry-standard benchmark HumanEval-x, and the specially designed CodeFuseEval for Chinese prompts. To assess the effectiveness of CodeFuse, we actively collected valuable human feedback from the AntGroup's software development process where CodeFuse has been successfully deployed. The results demonstrate that CodeFuse-13B achieves a HumanEval pass@1 score of 37.10%, positioning it as one of the top multi-lingual code LLMs with similar parameter sizes. In practical scenarios, such as code generation, code translation, code comments, and testcase generation, CodeFuse performs better than other models when confronted with Chinese prompts.

==> list.chineseexample.tex <==
\begin{figure*}
\lstset{frame=lrtb,
  language=python,
  aboveskip=3mm,
  belowskip=3mm,
  xleftmargin=2mm,
  xrightmargin=2mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small},
  % numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  % commentstyle=\color{teal},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=2,
  escapeinside={(*@}{@*)},
}

\begin{subfigure}{0.46\textwidth}
\begin{lstlisting}
% <|role_start|>human<|role_end|>
# (*@  \begin{CJK*}{UTF8}{gbsn}请用Java实现快排函数\end{CJK*} @*)
# Java
/**
 *  (*@\begin{CJK*}{UTF8}{gbsn}快速排序（挖坑法递归）\end{CJK*} @*)
 * @param arr   (*@\begin{CJK*}{UTF8}{gbsn}待排序数组\end{CJK*} @*)
 * @param low   (*@\begin{CJK*}{UTF8}{gbsn}左边界\end{CJK*} @*)
 * @param high  (*@\begin{CJK*}{UTF8}{gbsn}右边界\end{CJK*} @*)
 */
public static void sort(int arr[], int low, int high) {
    if (arr == null || arr.length <= 0) {
        return;
    }
    if (low >= high) {
        return;
    }

    int left = low;
    int right = high;
    int temp = arr[left]; //(*@\begin{CJK*}{UTF8}{gbsn}挖坑1：保存基准的值\end{CJK*} @*)

    while (left < right) {
        while (left < right && arr[right] >= temp) {
            right--;
        }
        arr[left] = arr[right]; //(*@\begin{CJK*}{UTF8}{gbsn}坑2：从后向前找到比基准小的元素，插入到基准位置坑1中\end{CJK*} @*)
        while (left < right && arr[left] <= temp) {
            left ++;
        }
        arr[right] = arr[left]; //(*@\begin{CJK*}{UTF8}{gbsn}坑3：从前往后找到比基准大的元素，放到刚才挖的坑2中\end{CJK*} @*)
    }
    arr[left] = temp; //(*@\begin{CJK*}{UTF8}{gbsn}基准值填补到坑3中，准备分治递归快排\end{CJK*} @*)
    System.out.println("Sorting: " + Arrays.toString(arr));
    sort(arr, low, left-1);
    sort(arr, left + 1, high);
}
\end{lstlisting}
% \vspace{-0.1in}
\subcaption{An example of code generation.}
\label{fig:cn_codegen_example}
\begin{lstlisting}
% <|role_start|>human<|role_end|>
# (*@  \begin{CJK*}{UTF8}{gbsn}请用Java翻译以下Python程序\end{CJK*} @*)
# Python
def sort_matrix(M):
    result = sorted(M, key=sum)
    return result
# Java
todo：
\end{lstlisting}
% \vspace{-0.1in}
\subcaption{An example of code translation.}
\label{fig:cn_codetrans_example}
\end{subfigure}
\begin{subfigure}{0.46\textwidth}
\begin{lstlisting}
% <|role_start|>human<|role_end|>
# (*@  \begin{CJK*}{UTF8}{gbsn}为以下Python代码生成单元测试\end{CJK*} @*)
# Python
from typing import List

def remove_duplicates(numbers: List[int]) -> List[int]:
    import collections
    c = collections.Counter(numbers)
    return [n for n in numbers if c[n] <= 1]
    
# Python
import unittest
from remove_duplicates import remove_duplicates

class TestRemoveDuplicates(unittest.TestCase):

    def test_remove_duplicates(self):
        numbers = [1, 2, 2, 3, 4, 4, 4, 5]
        expected_result = [1, 3, 5]
        result = remove_duplicates(numbers)
        self.assertEqual(result, expected_result)

    def test_remove_duplicates_empty_list(self):
        numbers = []
        expected_result = []
        result = remove_duplicates(numbers)
        self.assertEqual(result, expected_result)


if __name__ == '__main__':
    unittest.main()
\end{lstlisting}
% \vspace{-0.1in}
\subcaption{An example of testcase generation.}
\label{fig:cn_testcase_example}
\end{subfigure}

% \end{minipage}
\caption{Examples of \codefuse generation with prompts in Chinese. Prompt and generated codes are separated by multiple '#'s (added after the generation as an indicator).}
\end{figure*}

==> list.snippet.tex <==
\begin{figure*}
% \begin{minipage}[ht]{1\linewidth}
% \centering
% \newfontfamily\cjk{Code2000}
% \setmainfont{CODE2000.TTF}

\lstset{frame=lrtb,
  language=JSON,
  aboveskip=3mm,
  belowskip=3mm,
  xleftmargin=2mm,
  xrightmargin=2mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small},
  % numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=2,
  escapeinside={(*@}{@*)},
}
\begin{lstlisting}
{
    <|role_start|>human<|role_end|># Translate the following Python program to Java
# Python
def sort_matrix(M):
    result = sorted(M, key=sum)
    return result
# Java
    "prompt_text_chinese": (*@  \begin{CJK*}{UTF8}{gbsn}检查在给定的数字列表中，是否有任何两个数字比给定的阈值更接近。\end{CJK*} @*)
}
\end{lstlisting}
% \end{minipage}
\caption{An example from the expanded \humaneval dataset for the Python language.}
\end{figure*}

% \begin{figure*}
% % \begin{minipage}[ht]{1\linewidth}
% % \centering
% % \newfontfamily\cjk{Code2000}
% % \setmainfont{CODE2000.TTF}

% \lstset{frame=lrtb,
%   language=JSON,
%   aboveskip=3mm,
%   belowskip=3mm,
%   xleftmargin=2mm,
%   xrightmargin=2mm,
%   showstringspaces=false,
%   columns=flexible,
%   basicstyle={\small},
%   % numbers=left,
%   numberstyle=\tiny\color{gray},
%   keywordstyle=\color{blue},
%   commentstyle=\color{dkgreen},
%   stringstyle=\color{mauve},
%   breaklines=true,
%   breakatwhitespace=true,
%   tabsize=2,
%   escapeinside={(*@}{@*)},
% }
% \begin{lstlisting}
% {
%     "task_id": "Python/0",
%     "prompt": "from typing import List\n\n\ndef has_close_elements(numbers: List[float], threshold: float) -> bool:\n    \"\"\" Check if in given list of numbers, are any two numbers closer to each other than\n    given threshold.\n    >>> has_close_elements([1.0, 2.0, 3.0], 0.5)\n    False\n    >>> has_close_elements([1.0, 2.8, 3.0, 4.0, 5.0, 2.0], 0.3)\n    True\n    \"\"\"\n",
%     "canonical_solution": "    for idx, elem in enumerate(numbers):\n        for idx2, elem2 in enumerate(numbers):\n            if idx != idx2:\n                distance = abs(elem - elem2)\n                if distance < threshold:\n                    return True\n\n    return False\n",
%     "test": "\n\nMETADATA = {\n    'author': 'jt',\n    'dataset': 'test'\n}\n\n\ndef check(has_close_elements):\n    assert has_close_elements([1.0, 2.0, 3.9, 4.0, 5.0, 2.2], 0.3) == True\n    assert has_close_elements([1.0, 2.0, 3.9, 4.0, 5.0, 2.2], 0.05) == False\n    assert has_close_elements([1.0, 2.0, 5.9, 4.0, 5.0], 0.95) == True\n    assert has_close_elements([1.0, 2.0, 5.9, 4.0, 5.0], 0.8) == False\n    assert has_close_elements([1.0, 2.0, 3.0, 4.0, 5.0, 2.0], 0.1) == True\n    assert has_close_elements([1.1, 2.2, 3.1, 4.1, 5.1], 1.0) == True\n    assert has_close_elements([1.1, 2.2, 3.1, 4.1, 5.1], 0.5) == False\n\ncheck(has_close_elements)",
%     "text": "    Check if in given list of numbers, are any two numbers closer to each other than\n    given threshold.\n    >>> has_close_elements([1.0, 2.0, 3.0], 0.5)\n    False\n    >>> has_close_elements([1.0, 2.8, 3.0, 4.0, 5.0, 2.0], 0.3)\n    True",
%     "declaration": "from typing import List\n\n\ndef has_close_elements(numbers: List[float], threshold: float) -> bool:\n",
%     "example_test": "def check(has_close_elements):\n    assert has_close_elements([1.0, 2.0, 3.0], 0.5) == False\n    assert has_close_elements([1.0, 2.8, 3.0, 4.0, 5.0, 2.0], 0.3) == True\ncheck(has_close_elements)\n",
%     "prompt_text": "Check if in given list of numbers, are any two numbers closer to each other than given threshold.",
%     "prompt_explain": "Check if in given list of numbers, are any two numbers closer to each other than\ngiven threshold.\n>>> has_close_elements([1.0, 2.0, 3.0], 0.5)\nFalse\n>>> has_close_elements([1.0, 2.8, 3.0, 4.0, 5.0, 2.0], 0.3)\nTrue",
%     "func_title": "def has_close_elements(numbers: List[float], threshold: float) -> bool:",
%     "prompt_text_chinese": (*@  \begin{CJK*}{UTF8}{gbsn}检查在给定的数字列表中，是否有任何两个数字比给定的阈值更接近。\end{CJK*} @*)
% }
% \end{lstlisting}
% % \end{minipage}
% \caption{An example from the expanded \humaneval dataset for the Python language.}
% \end{figure*}

==> tab.chinese.tex <==
\begin{table}[ht]
  \caption{Evaluation of Chinese code comments and explanations on \codefuseeval and real feedback}
  \small
  \vspace{-1ex}
  \label{tab:chcc}
  \begin{tabular}{lcccc}
    \toprule
     {\textbf{Models}} & {\textbf{Bleu}}& {\textbf{BleuRT}}  \\ 
     
    % & & \textbf{Python}& \textbf{Java} & \textbf{C++} & \textbf{JavaScript} & \textbf{Go}  \\
    \midrule
\codefuse-13B-Base &	36.75\%&	27.76\%\\
%\codefuse-13B-SFT-V0&	36.75\%&	27.76\%\\
\codefuse-13B-SFT&	42.42\%&	36.34\%\\
%\codefuse-13B-MFT-DaLian&	37.46\%&	27.66\%\\
\bottomrule
\end{tabular}
\vspace{-1ex}
\end{table}


\begin{table}[ht]
  \caption{Evaluation of Chinese testcase generation on \codefuseeval}
\vspace{-1ex}
\small
  \label{tab:chtg}
  \begin{tabular}{lcc}
    \toprule
     {\textbf{Models}} & {\textbf{pass@1 Python}}& {\textbf{pass@1 Java}}  \\ 
    % & & \textbf{Python}& \textbf{Java} & \textbf{C++} & \textbf{JavaScript} & \textbf{Go}  \\
    \midrule
\codefuse-13B-SFT	&31.20\%	&24.32\% \\
\codegeex-13B	&22.89\%	&20.04\% \\
\bottomrule
\end{tabular}
\vspace{-1ex}
\end{table}






==> tab.mbppeval.tex <==
\begin{table}[ht]
  \caption{Comparing \codefuse's performance (pass@1) on \mbpp. \pengd{todo}
}
  \label{tab:mbpp}
  \begin{tabular}{lc}
    \toprule
     {\textbf{Models}} & {\textbf{\mbpp pass@1}}  \\ 
    % & & \textbf{Python}& \textbf{Java} & \textbf{C++} & \textbf{JavaScript} & \textbf{Go}  \\
    \midrule

CodeFuse-7B-SFT	&26.80\%\\
CodeFuse-13B-Pre-train &-\%\\
CodeFuse-13B-SFT-PLUS-Hello	&34.59\%\\
CodeFuse-13B-SFT-V1& -\%\\
CodeFuse-13B-SFT-Ant	&27.40\%\\
CodeFuse-13B-MFT-V1	&34.20\%\\
CodeFuse-13B-MFT-DaLian	&36.16\%\\
CodeFuse-13B(Open Source)&	35.6\%\\
CodeFuse-CodeLlama-34B(Open Source)&	-\%\\
\midrule

LLaMA-7B	&17.70\%\\
LaMDA-137B	&14.80\%\\
LLaMA-13B	&22.00\%\\
CodeGen-16B-Multi	&20.90\%\\
LLaMA-33B	&30.20\%\\
CodeGeeX-13B	&24.40\%\\
LLaMA-65B	&37.70\%\\
PaLM-540B	&36.80\%\\
CodeGen-16B-Mono	&35.30\%\\
StarCoderBase	&49.00\%\\
Code-cushman-001	&45.90\%\\
StarCoder-15.5B	&52.70\%\\
\bottomrule
\end{tabular}
\end{table}

